On Mobility Equity and the Promise of Emerging Transportation Systems

This paper introduces a mobility equity metric (MEM) for evaluating fairness and accessibility in multi-modal intelligent transportation systems. The MEM simultaneously accounts for service accessibility and transportation costs across different modes of transportation and social demographics. We provide a data-driven validation of the proposed MEM to characterize the impact of various parameters in the metric across cities in the U.S. We subsequently develop a routing framework that aims to optimize MEM within a transportation network containing both public transit and private vehicles. Within this framework, a system planner provides routing suggestions to vehicles across all modes of transportation to maximize MEM. We evaluate our approach through numerical simulations, analyzing the impact of travel demands and compliance of private vehicles. This work provides insights into designing transportation systems that are not only efficient but also equitable, ensuring fair access to essential services across diverse populations.

==> ref.tex <==
Brocker et al. \cite{brocker2010assessing} developed a spatial computable general equilibrium model to estimate the welfare effects and their spatial distribution resulting from transport infrastructure investments.
They evaluate project profitability, benefit spillovers across countries, and contributions to regional cohesion objectives.
As they focused on spatial distribution, there is lack of analysis for different societal groups.

% Such an accessibility to opportunities is essential for living a quality life \cite{mavoa2012gis}, especially transit accessibility for disadvantaged people. 
Mavoa et al. \cite{mavoa2012gis} introduced an accessibility index that is calculated based on the travel time of walking and taking public transit. Then, they combined the index with an average trip frequency of public transit to provide a more comprehensive picture of access in Auckland, New Zealand. The results highlighted the value of including service frequency in accessibility metrics.


El-Geneidy et al. \cite{el2016cost} proposed new accessibility measures that combine travel time and transit fare costs to better assess job accessibility by transit, especially for disadvantaged groups. Applying this to Montreal, Canada, the authors found that traditional time-based measures overestimate accessibility compared to the combined time/cost measures. Despite having higher overall accessibility, socially disadvantaged neighborhoods experienced a smaller loss in accessibility when accounting for fare costs compared to advantaged areas.

Mortazavi and Akbarzadeh \cite{mortazavi2017framework} developed a quantitative framework to assess transit equity using connectivity power with Gini index and car-less population as proxies for benefit and needs. Although this framework demonstrates how equity can be quantified for public transit, it has limitations, e.g., the analysis focuses on car-less citizens only and the framework is inapplicable to emerging mobility systems.

Jang et al. \cite{jang2017assessing} presented a quantitative approach to measure the spatial equity of transit provision in a city based on accessibility, applied it to assess equity levels for different transportation modes in Seoul, and demonstrated how planned network expansions (adding subway lanes) can improve spatial equity of public transportation across the urban area.
% This paper develops a methodology to calculate and analyze the spatial equity index of public transportation services in Seoul, South Korea using the Lorenz curve and Gini coefficient. The accessibility of subway stations and bus routes across the city's traffic analysis zones is estimated and weighted by service frequency. The spatial equity indices for subway and bus services are then calculated and compared, with subway found to be more unequally distributed than bus services. The impact of a planned new subway line extension on improving spatial equity is also assessed.
% The paper highlights the concept of spatial equity, defined as the horizontal equity or equal distribution of public transportation access across a city's geography and population. It contrasts this with vertical equity which considers distribution across different income/social groups.

Karner \cite{karner2018assessing} introduced a new route-level job-accessibility measure for assessing public transit equity, which can be calculated from public data.
Unlike the previous studies, this measure captures not only car-owner demographics but also demographics of other commuters to properly quantify how well the transit system provides job accessibility for different wage/income groups.
However, the analysis only considers commuting to employment locations, whereas transit dependent populations also rely on the system for accessing other types of destinations like healthcare, education, etc.
% This paper presents a method for assessing public transit service equity using route-level accessibility measures calculated from publicly available data sources like the General Transit Feed Specification (GTFS) and the U.S. Census Bureau's Longitudinal Employer-Household Dynamics (LEHD) dataset. The key differences from existing methods are:
% 1) It goes beyond just looking at the demographics of transit riders to consider how well the transit system provides accessibility to employment opportunities for different demographic groups.
% 2) It operates at the level of individual transit routes rather than just looking at system-wide averages, allowing for more nuanced equity analyses.
% 3) It uses highly disaggregate and temporally-specific transit travel time data from GTFS rather than relying on coarser transportation model outputs.
% 4) The accessibility measures link the locations of both employment opportunities and resident workers, providing a more complete picture than just considering job locations.

% In summary, the paper develops publicly available data-driven methods to quantify route-level employment accessibility by transit for different wage/income groups, aiming to better inform transit service equity analyses required by the Federal Transit Administration compared to current demographic-only approaches.

Pereira \cite{pereira2019future} estimated the accessibility impacts of the TransBrasil BRT project in Rio de Janeiro for different income groups using a cumulative opportunity measure under various travel time thresholds. The found that accessibility gains and their distribution across income levels are sensitive to the time threshold chosen. The study demonstrates how future scenario analysis can evaluate equity impacts of transport plans and highlights implications of the modifiable temporal unit problem. (This paper also considered jobs and public transit/walking)
% This paper analyzes how different scenarios of the TransBrasil BRT project in Rio de Janeiro, Brazil will likely impact the number of jobs accessible to the population of different income levels. The authors use a cumulative opportunity measure to estimate accessibility to jobs via public transport and walking under travel time thresholds of 30, 60, 90 and 120 minutes. They compare a business-as-usual baseline to two scenarios of partial and full implementation of the BRT project.
% The study finds that the full implementation of TransBrasil would lead to higher accessibility gains than the partial scenario, particularly for low-income groups, due to network effects of connecting the BRT to other transport modes. However, the size of the accessibility impacts and its distribution across income groups vary significantly depending on the travel time threshold chosen. The project would have more progressive and higher accessibility impacts for low-income groups under 30 or 60 minute thresholds, but more neutral and smaller impacts with 90 and 120 minute thresholds. 
% The main contributions are: 
% 1) Demonstrating how future scenario analysis can anticipate likely accessibility impacts of transport plans for different income groups
% 2) Showing that the conclusions of equity assessments of transportation projects can be sensitive to the time threshold chosen in cumulative opportunity measures, related to the modifiable temporal unit problem (MTUP).
% Limitations include focusing only on formal jobs, not considering long-term land use changes, and being limited to the municipality of Rio due to data constraints.


Cohn et al. \cite{cohn2019examining} investigated the potential impacts of autonomous vehicle (AV) adoption on transportation equity in the Washington, D.C. area.
To mimic the characteristics of an AV mode, they adjusted the system when AVs are introduced, e.g., increased roadway capacity, reduced terminal times, lowered parking costs, and shifts in the value of travel time and vehicle availability due to AV implementation. Additionally, the simulation method incorporates factors like increased discretionary trips and zero-occupancy trips.
While their results highlight potential benefits such as enhanced job accessibility for marginalized areas, they also identified concerning trends such as increased vehicle miles traveled and exposure to pollution, potentially exacerbating existing disparities. 
However, the results are directly derived from their modeling assumptions, which could potentially oversimplify the complexities of AV deployment and usage.
